Automatic Generation of Acceptance Test Cases from Use Case Specifications: an NLP-based Approach

Acceptance testing is a validation activity performed to ensure the conformance of software systems with respect to their functional requirements. In safety critical systems, it plays a crucial role since it is enforced by software standards. Test engineers need to identify all the representative test execution scenarios from requirements, determine the runtime conditions that trigger these scenarios, and finally provide the input data that satisfy these conditions. Given that requirements specifications are typically large and often provided in natural language, the generation of acceptance test cases tends to be expensive and error-prone. In this paper, we present UMTG, an approach that supports the generation of executable, system-level, acceptance test cases from requirements specifications in natural language, with the goal of reducing the manual effort required to generate test cases and ensuring requirements coverage. More specifically, UMTG automates the generation of acceptance test cases based on use case specifications and a domain model for the system under test, which are commonly produced in many development environments. Unlike existing approaches, it does not impose strong restrictions on the expressiveness of use case specifications. We rely on recent advances in natural language processing to automatically identify test scenarios and to generate formal constraints that capture conditions triggering the execution of the scenarios, thus enabling the generation of test data. In two industrial case studies, UMTG automatically and correctly translated 95% of the use case specification steps into formal constraints required for test data generation; furthermore, it generated test cases that exercise not only all the test scenarios manually implemented by experts, but also some critical scenarios not previously considered.

==> case_study.tex <==
\subsection{Industrial Case Studies}
\label{subsec:case_study}

We report our findings about the feasibility of our approach and its tool support in an industrial context. In order to experiment with \M{}~in multiple industrial projects, we applied it to ??? that we received from IEE.

\subsubsection{Goal}
\label{subsubsec:goall}
Our goal was to assess, in an industrial context, the feasibility of using  \M{}~to ???. 

\subsubsection{Study Context}
\label{subsubsec:study_context}
Study context...


\subsubsection{Results}
\label{subsubsec:case_study_results}
Case study results...

==> constraintIdentification.tex <==


\section{Identification of Constraints}
\label{sec:constraintIdentification}


The pre- and guard- conditions used in a use case specification capture the conditions under which 
a given use case scenario is executed, in other words they allow to determine the inputs that enable the covering of a given use case scenario. 
 \M{} automatically identifies these conditions by means of NLP and asks the software engineer 
 to reformulate them as OCL constraints. 
Since the execution of a scenario may depend also on how the system modifies its internal state, \M{} asks software engineers to specify with OCL the postconditions of the use case steps that represent internal operations. 
\M{} uses a constraint solver to solve the provided OCL constraints and automatically generate test inputs (see Section~\ref{sec:testGeneration}).

The postconditions of use case flows capture the expected state of the system after the  execution of the scenario. \M{} 
 asks the software engineer to reformulate postconditions of the use case flows as OCL constraints. 
 These postconditions are later translated into test oracles (see Section~\ref{sec:generationOfTestCases}).




\input{tableOCL}


To minimize manual effort, the NLP application first locates use case conditions and then identifies repeating and negated ones through an NLP transducer. If the use cases both feature a condition and its negation, software engineers are asked to reformulate only the condition as an OCL constraint. The negated OCL version of a constraint is automatically derived. Table~\ref{table:ocl} provides some of the use case conditions in Table~\ref{useCaseInitialOccupancy} with their corresponding OCL constraints based on the domain model. 







==> discussions.tex <==
\subsection{Discussions with the Engineers}
\label{subsec:discussions}
Discussions with the Engineers...

==> inputGeneration.tex <==
\section{Generation of Test Inputs} 
\label{sec:inputGeneration}


\M{} employs the Alloy analyzer~\cite{Jackson2006} to generate an object diagram (i.e., an instance of the domain model) in which the path condition in OCL holds for a given scenario. It leverages a model transformation that transforms OCL constraints into Alloy specifications~\cite{UML2Alloy}. %
Test input values are later extracted from the generated object diagram (see Section~\ref{sec:generationOfTestCases}).

We implemented an algorithm i.e., \emph{GenerateInputs} in Fig.~\ref{alg:testInputsGen}, which generates an object diagram for each test scenario of the input use case test model $tm$. %
To minimize the number of invocations of the constraint solver, we execute constraint solving only after all the test scenarios are identified (i.e., Lines~\ref{alg:inputs:invokingGenerateScenarios} and \ref{alg:inputs:solve} in Fig.~\ref{alg:testInputsGen}). %
What enables a minimal number of invocations of the constraint solver is function $unsatisfiable$ (Line~\ref{alg:ctg:allBranchesCovered} in Fig.~\ref{alg:testGen}), which returns false only if a path condition has been deemed unsatisfiable in a previous execution of the solver, otherwise it assumes that it can be solved thus letting \emph{GenerateScenarios} produce potentially infeasible scenarios.
Since some of the identified scenarios might be infeasible, we execute \emph{GenerateScenarios} multiple times, till all the branches have been covered or the number of iterations reaches a predefined threshold (Line~\ref{alg:inputs:until} in Fig.~\ref{alg:testInputsGen}). 



Unsatisfiable path conditions are usually with infeasible scenarios (i.e., scenarios which cannot be tested and verified by any set of possible input values).
In our context, we also observe unsatisfiable path conditions with feasible scenarios. These scenarios include an internal step that overrides the effects of the previous internal step.
For instance, in Scenario B in Fig.~\ref{fig:scenarioExamples}, the constraints 
\emph{C13} (i.e.,  {\scriptsize $\mathit{TemperatureLowError.allInstances()} \rightarrow \mathit{forAll(i} | \mathit{i.detected} = \mathit{true)}$}) and
\emph{C2} (i.e, {\scriptsize$\mathit{TemperatureError.allInstances()} \rightarrow \mathit{forAll(i} | \mathit{i.detected} = \mathit{false)}$} )
cannot be satisfied in the same path condition since \emph{TemperatureLowError} is a subclass of \emph{TemperatureError}.
The internal step with \emph{C13} (i.e., Line~\ref{uc2:af:resetTempLowError} in Table~\ref{useCaseInitialOccupancy}) sets a temperature error to \textit{detected} after the internal step with \emph{C2} (i.e., Line~\ref{uc2:af:setTempErrors} in Table~\ref{useCaseInitialOccupancy}) sets all the temperature errors to \textit{undetected}. %
 
 

 

\input{algos/generateInputs.tex} 

We first run the Alloy analyzer on each path condition, which returns object diagrams for satisfiable path conditions. 
We then incrementally run the Alloy analyzer on each unsatisfiable path condition to determine %
the ones with feasible scenarios. We identify the first constraint in the scenario that makes the path condition unsatisfiable. If this constraint belongs to an internal step (e.g., Scenario B in Fig.~\ref{fig:scenarioExamples}), then unsatisfiability depends on the redefinition of a variable; indeed, postconditions of internal steps characterize state updates (i.e., redefine variables) and thus cannot lead to unsatisfiable scenarios. Otherwise (i.e., if the constraint is a precondition of a use case or if it belongs to a conditional step), we consider the scenario infeasible. 

To enable automated constraint solving in the presence of variable redefinitions, we remove from the path condition the OCL constraints that characterize variables that have been redefined.
This is done by removing the constraints that precede the redefinition and appear in the unsat core\footnote{The unsat core is the minimal subset of OCL constraints that cannot be solved together~\cite{Torlak2008}, in our example C2 and C13.}  (i.e., C2 in our example). 
Since the removed constraints may, in principle, characterize an input value,
we keep track of the object diagram generated by the incremental solving procedure for later use (i.e., for the generation of the concrete inputs). However, usually, the removed constraints belong to internal steps that perform initial setups and thus do not have any effect on the identification of test inputs.  Constraint solving proceeds till the whole path condition is solved or the scenario is deemed infeasible.










==> oclFormat.tex <==

\subsection{Format of the Generated OCL Constraints}
\label{subsec:oclFormat}

The conditions described in the use case specifications of embedded systems are typically simple. For example, in \emph{BodySense}, the preconditions and condition steps describe safety checks ensuring that the environment has been properly set up (e.g., Line 2 in Table~\ref{table:ocl}) or that values have been properly derived (e.g., Line 6), while the internal steps describe the updates of state variables (e.g., Line 14).
These types of conditions can be expressed using the OCL according to the pattern in Fig.~\ref{fig:bnf}, which allows us to capture assignments, equalities, and inequalities. \M{} generates OCL constraints based on that pattern.





\begin{figure}
\scriptsize
\textbf{CONSTRAINT} = \textbf{CLASS} .allInstances() \textbf{[SELECTION]} 
          .forAll( \textbf{EXPR} )\\
\textbf{EXPR} = i $|$ i.\textbf{VARIABLE} \textbf{OPERATOR} \textbf{RHS} \\
\textbf{VARIABLE} = \textbf{ATTR} \textbf{$|$} \textbf{ASSOC}  \textbf{\{} .\textbf{ATTR} \textbf{$|$} \textbf{ASSOC} \textbf{\}}\\
\textbf{RHS} =  \textbf{VARIABLE} \textbf{$|$} \textbf{LITERAL};\\
\textbf{SELECTION} = $\rightarrow$ select( e $|$  \textbf{TYPESEL} \{ and \textbf{TYPESEL} \} )\\
\textbf{TYPESEL} = not e.TypeOf( \textbf{CLASS} ) \\
\textbf{Note:} This pattern is expressed using a simplified EBNF grammar~\cite{Ledgard:1980} where non-terminals are bold and terminals are not bold. \textbf{CLASS} stands for a class name appearing in the domain model, \textbf{LITERAL} is a OCL literal (e.g., '1' or 'a'), \textbf{ATTR} is an attribute of a class in the domain model, \textbf{ASSOC} is the name of an association end appearing in the domain model, \textbf{OPERATOR} is a math operator ( -, +,  =, $\textless$, $\le$, $\ge$, $\textgreater$).
\vspace{-3mm}
\caption{Pattern of OCL constraints generated by \M{}.}
\label{fig:bnf}
\end{figure}




The generated OCL constraints include a class name, an optional selection part, and an expression that should hold for all the
object instances \texttt{i} belonging to the selection (e.g., all the instances of the class).
The expression contains a left-hand side variable, an OCL operator, and a right-hand side term (either another variable or a literal).  
The optional selection part simply selects a subset of all the available instances based on the subtypes of the class \texttt{CLASS}.






==> questionnaire_study.tex <==
\subsection{Questionnaire Study}
\label{subsec:questionnaire}

We conducted a questionnaire study to evaluate, based on the viewpoints of the IEE engineers, how well our approach addresses the challenges that we identified in generating system test cases from use case specifications. The study is described and reported according to the template provided by Oppenheim et al.~\cite{Oppenheim1966}. 

\subsubsection{Planning and Design}
\label{subsubsec:planning}
Planning...

\subsubsection{Results and Analysis}
\label{subsubsec:resultsandanalysis}

Results and analysis...

==> scenarioGeneration.tex <==
\section{Generation of Test Scenarios} %
\label{sec:testGeneration}


\M{} generates, from a use case test model, a set of test scenarios which cover all the branches of the model (Step 8 in Fig.~\ref{fig:approach}). 
A scenario is a path in the use case test model that begins with a \emph{UseCaseStart} instance and ends with an \emph{Exit} or \emph{Abort} instance. 
It captures the sequence of interactions that should be stressed by its test case. 

\UMTG needs to identify test inputs in which the conditions in the scenario hold. %
For example, to test the scenario for the basic flow of the use case \emph{Classify Occupancy Status}, we need test inputs in which the capacitance value is above 600 (see Line~\ref{uc3:bf:capacitance} in Table~\ref{useCaseClassify}).   
We use the term \emph{path condition} to indicate a formula that conjoins all the conditions in a given scenario. 
If a path condition is satisfiable, we derive an object diagram (i.e., an instance of the domain model in which the path condition holds). 
For a given scenario, the test input values are extracted from the object diagram that satisfies the path condition. The rest of this section describes the test scenario generation algorithm while we provide the details of the test input generation in Section~\ref{sec:inputGeneration}.









We implemented an algorithm, i.e., \emph{GenerateScenario} in Fig.~\ref{alg:testGen}, 
which performs a recursive, depth-first traversal of a use case test model to generate test scenarios. 
It takes as input a use case test model (\emph{tm}),
a node to be traversed (\inst), 
a list of nodes (\emph{Scenario}) which contains the nodes of the same path traversed during the execution of \emph{GenerateScenario}, 
and an OCL constraint (\emph{pc}) which represents the path condition of the current scenario.
It generates a list of pairs $\langle Scenario, pc \rangle$ where each pair represents an OCL constraint of the path condition $pc$ for $Scenario$.  

\input{algos/generateScenarios}


\begin{figure*}[t]
  \centering
    \includegraphics[width=18cm]{images/scenarioExamples}
    \vspace{-3mm}
      \caption{Two scenarios built by \M{} when generating test cases for the use case 'Identify Occupancy Status' in Table~\ref{useCaseInitialOccupancy}.}
      \vspace{-3mm}
      \label{fig:scenarioExamples}
\end{figure*}  

Before calling \emph{GenerateScenario}, the use case test model $tm$ is merged with the use case test models of the included use cases in a way similar to the generation of interprocedural control flow graphs~\cite{Harrold-InterproceduralControlFlowGraph-ISSTA-1998}. The \emph{Include} instances in $tm$ are replaced with the \emph{UseCaseStart} instances of the included use cases; the \emph{Exit} instances of the basic flows of the included use cases are linked to the \emph{Node} instances following the \emph{Include} instances in $tm$.


We invoke \emph{GenerateScenario} with \inst being the \emph{UseCaseStart} instance in $tm$, %
\emph{Scenario} being an empty list, and \emph{pc} being an \emph{empty} constraint. Fig.~\ref{fig:scenarioExamples} shows two scenarios generated from the use case test model in Fig.~\ref{fig:testingModelExample}. %
Scenario A in Fig.~\ref{fig:scenarioExamples} covers, without taking any alternative flow, the basic flow of the use case \emph{Identify Occupancy Status} and the basic flows of the included use cases \emph{Self Diagnosis} and \emph{Classify Occupancy Status} in Table~\ref{useCaseInitialOccupancy}. Scenario B takes three specific alternative flows of the use cases \emph{Self Diagnosis}, \emph{Classify Occupancy Status} and \emph{Identify Occupancy Status}, respectively (Lines~\ref{uc2:af3:start} to~\ref{uc2:af3:post}, \ref{uc3:af3:start} to~\ref{uc3:af3:post}, and \ref{uc1:sat:start} to~\ref{uc1:sat:post} in Table~\ref{useCaseInitialOccupancy}). 



The precondition of the \emph{UseCaseStart} instance is added to the path condition for the initialisation of the test case (Lines~\ref{alg:ctg:initial}~to~\ref{alg:ctg:initialEnd} in Fig.~\ref{alg:testGen}). The \textit{Input} instances have no constraint to be added to the path condition (Lines~\ref{alg:ctg:input} to~\ref{alg:ctg:inputEnd}). We recursively call \emph{GenerateScenario} for the nodes following the \emph{UseCaseStart} and \emph{Input} instances (Lines~\ref{alg:ctg:start_generatescen} and~\ref{alg:ctg:input_generatescen}). For instance, Scenario A in Fig.~\ref{fig:scenarioExamples} starts with the \emph{UseCaseStart} instance of the use case \emph{Identify Occupancy Status} followed by an \emph{Input} instance, and proceeds with the \emph{UseCaseStart} instance of the included use case \emph{Self Diagnosis}. 

For each \emph{Condition} instance which is not \emph{InterruptingCondition}, we first visit the true branch and then the false branch to give priority to nominal scenarios (Lines~\ref{alg:ctg:condStart} to~\ref{alg:ctg:condEnd}). Bounded and global alternative flows are taken in the true branch of their \emph{InterruptingCondition} instances. 
Therefore, we first visit the false branch for the \emph{InterruptingCondition} instances %
(Lines~\ref{alg:ctg:intCondStart} to~\ref{alg:ctg:intCondEnd}). %
The condition of a bounded or global alternative flow is taken into account for the scenarios in which the alternative flow is taken. Therefore, we update the path condition for each condition branch except the false branch of the \emph{InterruptingCondition} instances (Lines~\ref{alg:ctg:compose1}, \ref{alg:ctg:neg2} and~\ref{alg:ctg:compose3}). For instance, Scenarios A and B do not cover the condition of the bounded alternative flow of the use case \emph{Identify Occupancy Status}. We recursively call \emph{GenerateScenario} for each branch (Lines~\ref{alg:ctg:followTrueGen}, \ref{alg:ctg:followFalseGen},~\ref{alg:ctg:followFalseGenIC} and~\ref{alg:ctg:followTrueGenIC}).


  



 

    
 







The \emph{Internal} instances represent the use case steps in which the system alters its state. Since state changes may affect the truth value of the following \emph{Condition} instances, the postconditions associated with the visited \emph{Internal} instances are added to the path condition (Line~\ref{alg:ctg:internalPC}). %
We recursively call \emph{GenerateScenario} for the nodes following the \emph{Internal} instances (Line~\ref{alg:ctg:generate}).

To avoid cycles in the generated scenarios, we proceed with the nodes following the \emph{Exit} instances only if the nodes have not been visited in the current scenario (Lines~\ref{alg:ctg:exitIncluded} and~\ref{alg:ctg:noLoop}).
An \emph{Exit} instance followed by a node represents either a resume step or a final step of an included use case.
An \emph{Exit} or \emph{Abort} instance which is not followed by any node indicates the termination of a use case. %
When the current scenario ends, we add the current scenario and its path condition to the set of scenario and path condition pairs to be returned (Line~\ref{alg:ctg:addTest}). %
For instance, Scenario A terminates with the \emph{Exit} instance of the basic flow of the use case \emph{Identify Occupancy Status}, while Scenario B terminates with the \emph{Abort} instance of the first specific alternative flow of the same use case.

The algorithm terminates when all the branches of the use case test model have been covered (Lines~\ref{alg:ctg:allBranchesCovered} to \ref{alg:ctg:allBranchesCoveredEndIF}) or all the edges have been visited. The depth-first traversal ensures that all the edges have been visited at least once.
The algorithm is guided towards the generation of scenarios with a satisfiable path condition (Lines~\ref{alg:ctg:UNSAT} to \ref{alg:ctg:UNSATEndIF}). 








==> tableOCL.tex <==
\begin{table*}[ht!]
\scriptsize
\caption{Some constraints for the use case `\textit{Identify Initial Occupancy Status of a Seat}'.}
\begin{center}
\begin{tabular}{|@{\hspace{0.10cm}}p{0.15cm}|@{\hspace{0.05cm}}p{3.8cm} |@{\hspace{0.05cm}}p{13.0cm} |}
\hline
\#&\textbf{Condition in the Use Case}&\textbf{Corresponding OCL Constraint}\\
\hline
C1&
the occupant class for airbag& 
$BodySenseSystem.allInstances()$\\
&control is valid&$\hskip 2em \rightarrow forAll(b | b.occupancyStatus.occupantClassForAirbagControl \tiny{\textless \textgreater} OccupantClass::Error )$
\\
\hline
C2&
the occupant class for seat belt&
$BodySenseSystem.allInstances()$\\
&reminder is valid&$\hskip 2em \rightarrow forAll(b | b.occupancyStatus.occupantClassForSeatBeltReminder \tiny{\textless \textgreater} OccupantClass::Error )$
\\
\hline
C3&
voltage error is detected&
$Error.allInstances() \rightarrow select(e | e.oclIsKindOf(VoltageError)) \rightarrow forAll(v|v.detected=true)$
\\
\hline
C4&the occupant classes for airbag&
$AirbagControlUnit.allInstances() \rightarrow forAll(a|a.status = a.bodySense.occupancyStatus$\\
&control and seat belt reminder&\hskip 2em $.occupantClassForAirbagControl)\ AND\  SeatBeltControlUnit.allInstances() $\\
&have been sent &$\hskip 2em  \rightarrow forAll(s|s.status = s.bodySense.occupancyStatus.occupantClassForSeatBeltReminder)$ \\
\hline
C5&
The system has been initialized
&
$BodySenseSystem.allInstances() \rightarrow forAll(b | b.initialized = true )$\\
\hline
C6&The system resets classification&$BodySenseSystem.allInstances()\rightarrow forAll(b | b.occupancyStatus.occupantClassForSeatBeltReminder $\\
&filters&$\hskip 2em  = null\  AND\ b.occupancyStatus.occupantClassForAirbagControl  = null)$\\
\hline
\end{tabular}
\end{center}
\label{table:ocl}
\end{table*}%






==> tableOCL2.tex <==
\begin{table*}[ht!]
\scriptsize
\caption{Some constraints for the use case `\textit{Identify Initial Occupancy Status of a Seat}'.}
\begin{center}
\begin{tabular}{|@{\hspace{0.05cm}}p{0.4cm}|@{\hspace{0.05cm}}p{3.8cm} |@{\hspace{0.05cm}}p{13.0cm} |}
\hline
Line &\textbf{Condition in the Use Case}&\textbf{Corresponding OCL Constraint}\\
\hline
2&
The system has been initialized
&
$\mathit{BodySense.allInstances()} \rightarrow \mathit{forAll(b} | \mathit{b.initialized} = \mathit{true} \mathit{)}$
\\
\hline
6&
the occupant class for airbag& 
$\mathit{BodySense.allInstances()}$\\
&control is valid&$\hskip 2em \rightarrow \mathit{forAll(b} | \mathit{b.occupancyStatus.occupantClassForAirbagControl} \tiny{\textless \textgreater} \mathit{OccupantClass::Error )}$
\\
\hline
13&
voltage error is detected&
$\mathit{VoltageError.allInstances()} \rightarrow \mathit{forAll(v}|\mathit{v.detected}=\mathit{true)}$
\\
\hline
14&
The system resets classification filters&$\mathit{BodySense.allInstances()}\rightarrow \mathit{forAll(b} | \mathit{b.occupancyStatus.occupantClassForAirbagControl}  = \mathit{null})$\\
\hline
\end{tabular}
\end{center}
\label{table:ocl}
\vspace{-5mm}
\end{table*}%






==> transformationRules.tex <==

\subsection{Transformation Rules}
\label{subsec:transformationRules}

\M{} implements a set of verb-specific transformation rules that enable the automated generation of OCL constraints from use case steps. %
The rules share a common structure and execute a predefined set of activities. %
Each rule is associated with a set of English verbs and is executed if one of the verbs appears in the use case step to process. 

In Section~\ref{subsec:gen}, we discuss to what extent we cover the verbs of the English language. In the following, we focus on the rules for the verbs \emph{to be}, \emph{to set}, and \emph{to enable}.


\input{algoTransf.tex}

Fig.~\ref{fig:alg:transform} shows the common algorithmic steps followed by the transformation rules. %
The rules rely on SRL roles to identify the left-hand side variables (hereafter lhs-variables), the operators, and the right-hand side terms (hereafter rhs-terms). For example, the phrases tagged with the role A1 are usually used to determine the variable on the left-hand side of an OCL expression.


The rules identify a set of variables that might be used on the left-hand side of the OCL expression (Line~\ref{algo:tranform:lhss} in Fig.~\ref{fig:alg:transform}). 
Instead of identifying a single variable for each OCL constraint to be generated, we opted for identifying a set of potential variables to be used for generating a set of OCL constraints in which we select the one with the highest score. 


The algorithm iterates over the lhs-variables to generate a distinct OCL constraint for each one (Lines \ref{algo:tranform:lhsFor} to \ref{algo:tranform:lhsForEnd} in Fig.~\ref{fig:alg:transform}). 
However, if the operator or the rhs-term of the OCL expression is not identified,
then the constraint is not generated (Line~\ref{algo:tranform:checkNull}).
If all the required elements are available, then the algorithm builds the OCL constraint according to the pattern in Fig.~\ref{fig:bnf} (Line~\ref{algo:tranform:build} in Fig.~\ref{fig:alg:transform}) and calculates the associated score (Line~\ref{algo:tranform:scoreCall}). Section~\ref{subsec:scoring} provides details of the formula used to calculate the score.

In addition to the rules for the different verbs that can appear in use case steps, \M{} includes a general transformation rule that is applied for any verb. We call this \emph{meta-verb transformation rule}.
This rule is based on the observation that use case steps are often translated to OCL constraints whose lhs-variable is an attribute whose name matches the name of the verb (or they are similar). Additional details about this transformation rule are provided in the following subsections. For every use case step, we apply both the verb-specific transformation rule and the meta-verb transformation rule. %


Sections~\ref{subsec:lhs}~to~\ref{subsec:scoring} describe the details of the steps of the algorithm, i.e., identifying the lhs-variables, identifying the rhs-term, identifying the operators to appear in the OCL constraint, and finally scoring the generated constraints.





